Inductive Bias Extraction and Matching for LLM Prompts

The active research topic of prompt engineering makes it evident that LLMs are sensitive to small changes in prompt wording. A portion of this can be ascribed to the inductive bias that is present in the LLM. By using an LLM's output as a portion of its prompt, we can more easily create satisfactory wording for prompts. This has the effect of creating a prompt that matches the inductive bias in model. Empirically, we show that using this Inductive Bias Extraction and Matching strategy improves LLM Likert ratings used for classification by up to 19% and LLM Likert ratings used for ranking by up to 27%.

==> llm_conversations.tex <==
\subparagraph{User\\}

Imagine you have done some number of steps, and you are evaluating how
likely it is that a given goal is the objective of a sequence of steps.
Design a fine grained 10 point scale for rating the likelihood that the
goal is the objective of the sequence of steps where 10 represents the
highest degree of likelihood and 1 represents the lowest degree of
likelihood.


\subparagraph{Assistant\\}

To design a fine-grained 10-point scale for rating the likelihood that a
given goal is the objective of a sequence of steps, I'll consider
various factors that contribute to this likelihood. Here's a proposed
scale:

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\item
  \textbf{Unrelated (1)}: The sequence of steps has no apparent
  connection to the goal. The steps seem to be random or unrelated to
  the goal in any way.
\item
  \textbf{Coincidental (2)}: The sequence of steps might coincidentally
  lead to the goal, but it's highly unlikely. There's no clear
  connection or logical reasoning behind the steps.
\item
  \textbf{Remote possibility (3)}: There's a very small chance that the
  sequence of steps might lead to the goal. However, it's still unclear
  how the steps relate to the goal.
\item
  \textbf{Indirect connection (4)}: The sequence of steps has an
  indirect connection to the goal. The steps might be related to a
  broader context or a secondary goal, but it's not directly related to
  the primary goal.
\item
  \textbf{Possible intermediate step (5)}: The sequence of steps might
  be an intermediate step towards the goal, but it's not clear if it's a
  necessary or sufficient step.
\item
  \textbf{Probable intermediate step (6)}: The sequence of steps is
  likely an intermediate step towards the goal. The steps seem to be
  moving in the right direction, but there might be some missing links.
\item
  \textbf{Strong connection (7)}: The sequence of steps has a strong
  connection to the goal. The steps seem to be building towards the
  goal, and there's a clear logical progression.
\item
  \textbf{Highly likely (8)}: The sequence of steps is highly likely to
  be leading towards the goal. The steps are well-structured, and
  there's a clear path towards achieving the goal.
\item
  \textbf{Almost certain (9)}: The sequence of steps is almost certain
  to be leading towards the goal. The steps are well-defined, and
  there's a clear understanding of how they relate to the goal.
\item
  \textbf{Certain (10)}: The sequence of steps is definitely leading
  towards the goal. There's no doubt or ambiguity about the connection
  between the steps and the goal.
\end{enumerate}

This scale provides a fine-grained evaluation of the likelihood that a
given goal is the objective of a sequence of steps. It considers various
factors, such as the connection between the steps and the goal, the
logical progression, and the clarity of the path towards achieving the
goal.

\subparagraph{User\\}

For the following query, start your response with a rating from 1 to 10
using the previous scale that considers how likely a goal is the
objective of a sequence of steps. How likely is it that the goal
sentence ``Recover from the flu'' is the objective of the following
paragraph of steps? Sam got a cold one day. He tried to ignore it. But
it grew worse, so he went to the doctor. The doctor told Sam he had the
flu! Sam refused to take medicine and ended up developing a pneumonia.


\subparagraph{Assistant\\}

Rating: 1 (Unrelated)

The goal sentence ``Recover from the flu'' is not the objective of the
sequence of steps in the given paragraph. In fact, the sequence of steps
seems to be leading to the opposite outcome, where Sam's condition
worsens due to his refusal to take medicine, ultimately resulting in
pneumonia. The steps do not demonstrate any attempt to recover from the
flu, and the outcome is actually a deterioration of Sam's health.
Therefore, the likelihood of the goal being the objective of the
sequence of steps is extremely low, earning a rating of 1.

